A Systematic Survey on Event Camera Representation Learning

Event cameras offer distinctive advantages, including microsecond-level latency and high dynamic range, rendering them promising for challenging perception tasks. Inspired by biological vision, they output asynchronous and sparse event streams rather than dense image frames, creating a fundamental mismatch with mainstream neural networks. This survey reviews recent advances in event camera representation learning from the perspective of converting raw event streams into learnable representations. We first organize existing methods according to whether they rely on a single principal event representation or jointly exploit multiple complementary representations. Single-representation methods are further categorized into dense-based representations, which regularize events into structured grid-like forms, and sparse-based representations, which preserve event-native discrete spatio-temporal structures. Multi-representation methods are organized into dense-dense and dense-sparse hybrid formulations that exploit complementary representation properties. This representation-centric taxonomy clarifies how different paradigms balance structural regularity, temporal fidelity, sparsity preservation, and architectural compatibility. For each paradigm, we examine the underlying design choices, modeling principles, and task-level implications. We further summarize standard benchmarks and evaluation settings across representative high-level perception and low-level vision tasks. Finally, we discuss open problems and outline future directions from fixed representation design toward adaptive representation optimization, improved fidelity-efficiency trade-offs, and more scalable event-based perception systems.

==> sec/7_specific_representation.tex <==
\section{Specific Representation}

Beyond the conventional dichotomy between frame-based and point-based representational paradigms, contemporary research has pivoted toward developing tailored event representations that optimize the core information encoding pipeline. These advanced methodologies seek to overcome the inherent limitations of manual heuristic design by integrating automated optimization metrics, self-supervised learning paradigms, semantic decoupling strategies, and multi-view consistency constraints. By customizing the representation generation pipeline to align with the unique intrinsic properties of asynchronous event streams and the specific performance requirements of diverse downstream tasks, these approaches deliver enhanced performance and robustness in complex real-world scenarios.

In particular, to mitigate the prohibitive computational overhead associated with manual tuning of representation hyperparameters, Zubi\'{c} et al.~\cite{zubic2023chaos} proposed a dedicated metric-guided automated search framework. The authors introduce the Gromov-Wasserstein Discrepancy as an efficient and effective proxy metric to quantify the degree of structural alignment between the raw event graph and the corresponding dense grid-based representation. Rather than relying on resource-intensive neural network training for representation evaluation, the optimal representation parameters $p^*$ are derived directly by minimizing the expected optimal transport cost, formulated as follows:
\begin{equation}
    p^* = \mathop{\arg\min}_{p} \mathbb{E}_{\mathcal{E}} \left[ \mathcal{GW}(\mathcal{E}, \mathcal{R}_p(\mathcal{E})) \right],
\label{eq:gwd-optimization}
\end{equation}

\noindent where $\mathcal{GW}$ denotes the Gromov-Wasserstein discrepancy metric, $\mathcal{E}$ represents the raw asynchronous event stream, and $\mathcal{R}_p$ refers to the learnable representation function parameterized by hyperparameters $p$ (e.g., various event aggregation and binning strategies). This end-to-end automated optimization pipeline yields the discovery of ERGO-12, a novel multi-channel event representation that consistently outperforms conventional hand-crafted feature representations across standard evaluation benchmarks.


While the aforementioned work centers on automated hyperparameter optimization, parallel research efforts tackle the inherent noise and signal corruption present in raw event data via physics-guided representation learning paradigms. Qu et al.~\cite{qu2024evrepsl} introduced EvRepSL, a dedicated self-supervised framework designed to learn robust, noise-resilient event representations by explicitly modeling the underlying physical correlation between asynchronous event streams and synchronous intensity frames. The representation generation network is trained end-to-end in a self-supervised fashion, with the core objective of reconstructing the predicted intensity image $\hat{I}_{t_1}$ at timestamp $t_1$ from the reference intensity frame $I_{t_0}$ at an earlier timestamp $t_0$, supervised by the accumulated event polarity signal $\Sigma p$ (i.e., $\mathcal{E}_I$) and the learned parameters $\theta, k$. This physical reconstruction process is formalized via the following formulation:
\begin{equation}
    \hat{I}_{t_1}(\mathbf{u}) = \exp\left(\theta(\mathbf{u}) \cdot \Sigma p(\mathbf{u})\right) \cdot \left(I_{t_0}(\mathbf{u}) + k\right) - k,
\label{eq:evrepsl-physics}
\end{equation}

\noindent where $\mathbf{u}$ denotes the 2D pixel coordinate on the image plane, $\theta$ and $k$ represent learnable physical parameters corresponding to contrast sensitivity thresholds and intensity offset mapping factors, respectively. By embedding and enforcing this explicit physical imaging constraint throughout the training process, the network is able to generate clean, denoised event representations that effectively preserve spatial-temporal structural details, relying solely on raw event data during the inference stage without requiring auxiliary supervision.

Moving beyond dedicated noise reduction strategies, contemporary research has further shifted toward exploring and modeling the explicit semantic structure inherent in event representations. Drawing inspiration from the hierarchical processing mechanism of the human visual system, Chen et al.~\cite{chen2025motion} proposed a novel Motion and Appearance Decoupling representation paradigm tailored for asynchronous event data. To effectively disentangle the intertwined spatiotemporal information embedded within raw event streams, the authors construct a dedicated appearance tensor $\mathcal{T}_a$ by warping individual events to a unified global reference timestamp $t_{ref}$ guided by the estimated dense optical flow $\mathbf{v}_k$ for each event, with the formulation given as:
\begin{equation}
    \mathcal{T}_a(\mathbf{u}) = \sum_{k} \delta \left( \mathbf{u} - (\mathbf{u}_k + (t_{ref} - t_k)\mathbf{v}_k) \right),
\label{eq:mad-decoupling}
\end{equation}

\noindent where $\delta(\cdot)$ denotes the Dirac delta function used for event alignment and aggregation. This coarse-to-fine spatial-temporal alignment pipeline effectively eliminates motion-induced blur artifacts that commonly plague event-based representations, enabling the dedicated appearance branch to concentrate exclusively on extracting static texture and structural details. Concurrently, a complementary parallel branch is designed to explicitly encode independent motion dynamics and temporal cues, which substantially alleviates the feature learning burden for subsequent downstream tasks and boosts overall model convergence and performance.

Last but not least, recognizing that reliance on a single event representation inevitably incurs task-specific information loss and limited generalization, Zheng et al.~\cite{zheng2024eventdance} introduced a versatile multi-view representation strategy within their unified EventDance framework. This approach leverages multiple complementary and semantically distinct event representations in parallel, including canonical formats such as Voxel Grid, Stack Image, and Event Stack Tensor (EST). To fully harness the complementary information encoded across these diverse representations and enforce prediction coherence, the framework imposes a dedicated cross-representation consistency loss $\mathcal{L}_{cons}$ over the predictive distributions $P$ generated by separate branch-specific encoders, formulated as:
\begin{equation}
    \mathcal{L}_{cons} = \sum_{i \neq j} \mathcal{D}_{KL} \left( P(r_i(\mathcal{E})) \parallel P(r_j(\mathcal{E})) \right),
\label{eq:eventdance-consistency}
\end{equation}

\noindent where $r_i$ and $r_j$ denote distinct branch-wise representation functions corresponding to different encoding paradigms, and $\mathcal{D}_{KL}$ refers to the Kullback-Leibler divergence used to measure distribution discrepancy. This cross-consistency regularization mechanism effectively bridges the inherent modality gap between heterogeneous event representations, enhancing model stability and ensuring consistent, robust performance particularly in challenging unsupervised source-free adaptation scenarios where annotated source training data is completely unavailable.
